Causal-JEPA: Learning World Models through Object-Level Latent Masking

World models require robust relational understanding to support prediction, reasoning, and control. While object-centric representations provide a useful abstraction, they are not sufficient to capture interaction-dependent dynamics. We therefore propose C-JEPA, a simple and flexible object-centric world model that extends masked joint embedding prediction from image patches to object-centric representations. By masking object-level latents and requiring each masked object state to be inferred from the surrounding context, C-JEPA imposes structured partial observability during training, creating counterfactual-like prediction queries that discourage shortcut solutions and make interaction-dependent prediction necessary under the learning objective. Empirically, C-JEPA leads to consistent gains in visual question answering, with an absolute improvement of about 20% in counterfactual reasoning over the same architecture without object-level masking. On agent control tasks, C-JEPA enables substantially more efficient planning by using only 1% of the total latent input features required by patch-based world models, while achieving comparable performance. Finally, we provide a formal analysis demonstrating that object-level masking induces useful inductive bias by controlling observability. Our code is available at https://github.com/galilai-group/cjepa.

==> table/oc_worldmodels.tex <==
\begin{table*}[t!]
\ttabbox[]
  {\centering
   \tabcolsep=0.12cm
    \renewcommand{\arraystretch}{1}
    \small
\centering
\caption{Comparison of object-centric world models in terms of representation, interaction modeling, and learning objectives.}
\label{tab:ocwm_comparison}
\renewcommand{\arraystretch}{1.2}

\begin{tabular}{lccccc}
\toprule
\textbf{Model} 
& \textbf{Pixel / Feature Decoder} 
& \textbf{Interaction Inductive Bias} 
& \textbf{Supervision} \\
\midrule
FOCUS~\cite{32} 
& Yes 
& Reward-driven interaction exposure 
& Object masks  \\

Factorized WM~\cite{29} 
& Yes 
& Shared latent cause of transition 
& Object / actor masks \\

STICA~\cite{40} 
& Yes 
& Attention in policy/value networks 
& Self-supervised  \\

OCVP~\cite{2} 
& Yes 
& Attention-level factorization 
& Self-supervised  \\

SOLD~\cite{1} 
& Yes 
& Decoupled self / interaction dynamics 
& Self-supervised \\

SlotFormer~\cite{11} 
& Optional 
& Transformer self-attention 
& Self-supervised  \\

C-SWM~\cite{33} 
& No 
& Fixed graph (GNN) 
& Self-supervised \\

SPARTAN~\cite{3} 
& No 
& Sparse attention (architectural prior) 
& Self-supervised \\

\midrule
\textbf{C-JEPA (ours)} 
& \textbf{No} 
& \textbf{Object-level latent masking (objective-induced)} 
& \textbf{Self-supervised}  \\
\bottomrule
\end{tabular}
      }%
    {}%
\end{table*}%

